When AI Bends Metal: AI-Assisted Optimization of Design Parameters in Sheet Metal Forming

Numerical simulations have revolutionized the industrial design process by reducing prototyping costs, design iterations, and enabling product engineers to explore the design space more efficiently. However, the growing scale of simulations demands substantial expert knowledge, computational resources, and time. A key challenge is identifying input parameters that yield optimal results, as iterative simulations are costly and can have a large environmental impact. This paper presents an AI-assisted workflow that reduces expert involvement in parameter optimization through the use of Bayesian optimization. Furthermore, we present an active learning variant of the approach, assisting the expert if desired. A deep learning model provides an initial parameter estimate, from which the optimization cycle iteratively refines the design until a termination condition (e.g.,energy budget or iteration limit) is met. We demonstrate our approach, based on a sheet metal forming process, and show how it enables us to accelerate the exploration of the design space while reducing the need for expert involvement.

==> Makefile <==
# Default target
BASENAME ?= main

all: pdf

pdf: $(BASENAME).tex $(FIGURES) $(STYLEFILES)
	pdflatex -shell-escape $(BASENAME).tex
	bibtex $(BASENAME)
	# makeglossaries $(BASENAME)
	pdflatex -shell-escape $(BASENAME).tex
	pdflatex -shell-escape $(BASENAME).tex
	@echo "\033[91m\n\n---------------------------------------\033[0m"
	@echo "\033[92mtarget \033[91m$(BASENAME).pdf \033[92mfinished successfully\033[0m"
	@echo "\033[91m---------------------------------------\n\033[0m"

# 👇 NEW: IEEE target
ieee:
	$(MAKE) BASENAME=old_main_ieee pdf

# Optional explicit main target
main:
	$(MAKE) BASENAME=main pdf

clean:
	@rm -f *~ *.aux *.bbl *.blg *.dvi *.log *.pdfsync *.ps *.tpt *.tgz
	@rm -f main.pdf old_main_ieee.pdf
	@echo "\n\033[92mtarget clean finished\n\033[0m"

show:
	evince $(BASENAME).pdf

force:
	touch $(BASENAME).tex
	$(MAKE) pdf

AD: appendix

appendix: AD.pdf

AD.pdf: AD.tex
	pdflatex AD.tex

